Beamformed Energy Detection in the Presence of an Interferer for Cognitive mmWave Network

In this paper, we propose beamformed energy detection (BFED) spectrum sensing schemes for a single secondary user (SU) or a cognitive radio to detect a primary user (PU) transmission in the presence of an interferer. In the millimeter wave (mmWave) band, due to high attenuation, there are fewer multipaths, and the channel is sparse, giving rise to fewer directions of arrivals (DoAs). Sensing in only these paths instead of blind energy detection can reap significant benefits. An analog beamforming weight vector is designed such that the beamforming gain in the true DoAs of the PU signal is maximized while minimizing interference from the interferer. To demonstrate the bound on the system performance, the proposed sensing scheme is designed under the knowledge of full channel state information (CSI) at the SU for the PU-SU and Interferer-SU channels. However, as the CSI may not be available at the SU, another BFED sensing scheme is proposed, which only utilizes the estimate the DoAs. To model the estimates of DoAs, perturbations are added to the true DoAs. The distribution of the test statistic for BFED with full CSI schemes is derived under the null hypothesis so that the threshold of the Neyman-Pearson detector can be found analytically. The performance of both schemes is also compared with the traditional energy detector for multi-antenna systems.

==> Temp.tex <==
%----Temp Introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the recent past there has been tremendous increase in the traffic  due to rise in the demand of mobile devices, internet of things (IoT) devices and data based applications. One way to meet this requirement is moving to mmWave band, which provides large bandwidths. To improve on spectrum utilization in these bands,  cognitive radio will be  very helpful. Cognitive mmWave technology will be able to meet the demands \cite{mmWaveCR}.
%para 1 citation Physical Layer Security in Cognitive Millimeter Wave Networks

In cognitive radio technology, spectrum sensing plays a key role as it provides spectrum awareness required for cognitive processing.Several spectrum sensing techniques are proposed in literature mostly based on statistical hypothesis test.\cite{Thesis}
Energy detection is a simplest spectrum sensing technique suggested in literature. This technique is preferred as it does not require any a priori knowledge of the primary user (PU) signal.



%%%%%%%%% 3rd paragrah why consider interferer%%%%%%%%


%%%%%% 4th paragraph need for beamforming %%%%%%%%%%
In a mmWave system the signal undergoes severe propagation loss and travel in highly directional manner leading to fewer multipaths \cite{bfmg}.
In this system large number of antennas can be packed in a small form factor, thus giving beamforming gains  to overcome severe propagation loss.
In beamforming the signal from each antenna is given a phase shift to form a beam in the intended direction while having null in the unintended direction.
%A survey of millimeter wave communications (mmWave) for 5G:opportunities and challenges



%%%%Litreature survey%%%%%%%%%%

% ParaIII: Literature Survey on Beamforming based detection
\emph{Most of the beamforming methods in cognitive radio literature only consider transmit-beamforming to reduce the interference from secondary users (SUs) to the PUs \cite{beamforming_4_CR1, beamforming_4_CR2, beamforming_4_CR3}. %Although  simultaneous distributed and estimation based spectrum sharing is proposed in \cite{beamforming_4_CR4}, distributed detection is performed without beamforming while secondary user transmission is done using beamforming. 
The scope of this paper is different from the above papers on beamforming in cognitive radios as this paper focuses on receive-beamforming for spectrum sensing purposes using single user with multiple antennas. There have been only few papers on this topic \cite{ BF_Sensing_1, BF_Sensing_2}. In \cite{BF_Sensing_1}, eigenvalue-based spectrum sensing algorithm is proposed using beamformed received data. In \cite{BF_Sensing_2}, the angular domain is divided into sectors using beamforming and these sectors are then sensed serially. A electronically steerable parasitic antenna receptor is used for sensing so that only a single RF front end is required simplifying the cost, power and size requirements of the radio. }
SU user uses BFED to detect the presence of primary user in an AWGN channel\cite{NCC}.



%%%%%our contribution%%%%%%%%

In this paper we propose two methods for spectrum sensing. In the first method, perturbed beamformed energy detection (BFED), we assume that estimated DoAs of the signals from PU and interferer are available. Using these DoAs, an analog beamforming weight vector is designed such that the peaks in the radiation pattern are toward the PU direction and null in the interferer direction. \emph{Here DoA is not estimated, rather error is added using CRB}. BFED is performed by using the computed weight vector. In the second proposed method, perfect  full channel state information (CSI) BFED with  of both PU and interferer is available at the SU. Similar formulation is used here to design the weight vector as in the above method. This method is proposed to show the performance difference achieved between both the methods. 



% ParaV: Organization of this paper
The paper is organized as follows. Section II presents the system model followed by basics of ED in Section III. Section IV and section V presents the details of the proposed methods, perturbed BFED  and perfect CSI BFED. Section V presents simulation results while Section VI concludes the paper. 




%additive white Gaussian noise (AWGN).   

%\textcolor{red}{Markafi2012}In this paper, we also seek to analyse the performance of asingle spectrum sensing node by taking into account the intra-network interference generated by the secondary network.This is justified when the CR nodes are non cooperating and not synchronized, such that a few secondary users (SU)1arenot silent while others are sensing the spectrum. This meansall CR nodes do not commence and terminate sensing andtransmission simultaneously. 

 %\textcolor{red}{Lagunas2014}In practical Cognitive Radio (CR) networks, primary users must be detected even in the presence of low-regulated transmissions from unlicensed systems, which cannot be taken into account in the CS model because of their non-regulated nature.

%\cite{Lagunas2014}: Extraction of the primary user frequency locations is then performed based on sparse signal recovery algorithms in the presence of interference.
%This paper compares different CS-based reconstruction strategies for extraction of primary user frequency location in CR. Unlike other works, the proposed model considers the existence of interferences emanating from low-regulated transmissions, which cannot be taken into account in the CS model because of their non-regulated nature.

